DANAE: a denoising autoencoder for underwater attitude estimation

One of the main issues for underwater robots navigation is their accurate positioning, which heavily depends on the orientation estimation phase. The systems employed to this scope are affected by different noise typologies, mainly related to the sensors and to the irregular noise of the underwater environment. Filtering algorithms can reduce their effect if opportunely configured, but this process usually requires fine techniques and time. In this paper we propose DANAE, a deep Denoising AutoeNcoder for Attitude Estimation which works on Kalman filter IMU/AHRS data integration with the aim of reducing any kind of noise, independently of its nature. This deep learning-based architecture showed to be robust and reliable, significantly improving the Kalman filter results. Further tests could make this method suitable for real-time applications on navigation tasks.

==> orient.tex <==
The orientation of an object is easily understood as the set of rotations that relates the object coordinates system to the one taken as reference. The most used parameterizations are the Euler angles, and their analogous, Tait-Bryan angles, rotation vectors, rotation matrices, and unit quaternions \cite{bernal2017orientation}. A detailed survey of this representation can be found in \cite{shuster1993survey}. For the purposes of our study, some notions on reference systems and eulerian representations are given. 
While localization is defined with respect to a global reference frame, vehicles IMUs generally refer their attitude to the local East-North-Up (ENU) or the North-East-Down (NED) coordinate frames. The latter is mainly adopted for underwater applications: the positive X-axis points to the North, the positive Y-axis to the East, and the positive Z-axis follows the positive direction of the gravity force. Other custom body frames can be adopted when acquiring data from sensors, so it is of fundamental importance to specify this configuration in order to properly transform the measurements in the correct frame. A perfect example in this sense comes from the Matlab Mobile application for smartphones \cite{MatlabOR}: in this custom body frame the positive X-axis and Y-axis extend out of the right and of the top side of the smartphone respectively, while the positive Z-axis points out of the front face of the phone, independently of the actual configuration. With this state, the Euler angles are defined as follows:
\begin{itemize}
	\item $\phi$ represents the rotation around the X axis, known as roll.
	\item $\theta$ defines the rotation around the Y axis, that is the pitch angle.
	\item $\psi$ is related to the yaw angle around the Z axis.
\end{itemize}

==> pezzi_di_testo.tex <==
Another interesting approach is
based on the KF to estimate the sensors signals
noise or their biases, since they can heavily affect
the final estimation [Embedded Kalman Filter For
Inertial Measurement Unit (IMU) on the
Atmega8535]. However, due to the high precision
and reliability requirements it has to satisfy, these
systems are generally costly and unaffordable for
small-scale robots. Newly developed Attitude and
Heading Reference System (AHRS) can equally
provide very satisfying results, integrating the
magnetometer to the IMU configuration. The
progresses made with these technologies made
AHRS one of the most popular low-cost attitude
sensor for robots, especially in underwater
environments. However, even in this case sensors
misalignment, biases and other disturbance factors
can lead to noisy or deviated values and impact on
the vehicle positioning [Application of Modified EKF
Based on Intelligent Data Fusion in AUV Navigation]
Kalman filtering-based techniques constitute a
powerful approach to this problem since they allow
to estimate both the state and the sensors biases,
while the noise matrices expressing the covariance
of the measurements and of the process can be fine
tuned to reduce as much as possible the noise
influence. However, it presents some drawbacks. An
example is that it requires on-line computation of the
error covariance matrix for any time-varying or
nonlinear system, squaring the number of necessary
updating step at each time. Moreover, the formal nature of the Kalman filter makes the tuning phase a
nonintuitive other than not easy process [An Intuitive
Approach to Inertial Sensor Bias Estimation].
In summary, any kind of external factor combined
with the internal difficulties related to the sensors
integration can bring angle errors. A not accurate
angles estimation (especially the heading one) will
inevitably impact on the performance of the vehicle
[Shallow-sea application of an intelligent fusion
module for low-cost sensors in AUV].
In the past few years, Deep Learning (DL) gained
a huge scientific interest, making progresses in
Natural Language Processing (NLP) and computer
vision tasks. Convolutional Neural Networks (CNN),
Recurrent Neural Networks (RNN) and
Reinforcement Learning (RL) are the principal deep
neural networks, used to successfully accomplish
several tasks in the most disparate fields
[Application of Modified EKF Based on Intelligent
Data Fusion in AUV Navigation]. For example,
unsupervised feature learning for single modalities
(such as text or audio) have recently been
developed. In this case, a deep denoising
autoencoder is trained to predict the original clean
audio feature from deteriorated one, and then
processed to conduct an isolated word recognition
task [Audio-visual speech recognition using deep
learning]. Expanding these concepts, an intelligent
deep denoising autoencoder is proposed to improve
the Kalman filter outputs, significantly reducing the
difficulties related to the parameters tuning, the
biases definition and the effects of other noise
sources. The strength of this method stands in the
development of a full-noise compensation model,
without the needs to separately process each
influencing factors.

%% PEZZI DI RELATED WORKS:
 The course heading angles which are
obtained from GPS rather than the vehicle heading angles
are treated as the truth heading angles for training the
full-noise model, because the course heading angles from
GPS are the resultant heading angles which are generated
by vehicle heading angles and all the other influencing
factors on heading angles, such as magnetic interference
and water current. This is why GPS heading angles rather
than vehicle heading angles are selected as the truth
heading angles both in the module and in the following
comparison.
This paper [Attitude Estimation Using Kalman
Filtering: External Acceleration Compensation
Considerations] paper proposes extended Kalman filter-
based attitude estimation using a new algorithm to
overcome the external acceleration. This algorithm is
based on an external acceleration compensation model to
be used as a modifying parameter in adjusting the
measurement noise covariance matrix of the extended
Kalman filter.The experiment was conducted to verify the
estimation accuracy, that is, one-axis andmultiple axes
sensormovement. Five approacheswere used to test the
estimation of the attitude: (1) theKF-based model without
compensating for external acceleration, (2) the
proposed KF-based model which employs the external
acceleration compensation model, (3) the two-step KF
using weighted-based switching approach, (4) the KF-
based model which uses the threshold-based approach,
and (5) the KF-based model which uses the threshold-
based approach combined with a softened part approach.
The proposed algorithm showed high effectiveness
during the one-axis test. When the testing conditions
employed multiple axes, the estimation accuracy
increased using the proposed approach and exhibited
external acceleration rejection at the right timing. The
proposed algorithm has fewer parameters that need to be
set at the expense of the sharpness of signal edge
transition.



For example, Robert B. Smith et al. (2003)
proposed a three-axis algebraic model which is
used to numerically compensate  for magnetic errors
by only measuring magnetic field values. Similarity,
a temperature compensation method was presented
by Qiang Fu for the MEMS accelerometer in the
AHRS (Qiang et al., 2009).
Different from these methods, we
propose an intelligent fusion module which focuses on seeking out the full-noise model instead of
compensating for low-cost sensors. The intelligent
fusion module not only takes sensors' error into
account, but also external environment.  OP-ELM has been
demonstrated to be more suitable to generate the
intelligent fusion module for AUV in this paper. In
this paper, we take heading angles which are from
digital compass or AHRS for example. Because
some circumstance such as strong magnetic or
violent acceleration/deceleration may cause
untrustworthy data for sensors, we judge status of
sensors' data and adopt different full-noise models
which are obtained by OP-ELM for credible sensors'
data in the intelligent fusion module. 
\cite{guo2018shallow} propose
an intelligent fusion module to obtain
the full-noise model for AUV. By combining full-noise model with credible data by
using OP-ELM to improve the accuracy of positioning
and navigation. Our method has been demonstrated by a
range of real data, which RMSE can at most improve by
86.4percent in complex conditions than Extended Kalman
Filter' AUV, which need to go to explore the unknown
area, is impossible to obtain the exact location of
the magnetic interference substance. For AHRS, it has
the problem of accumulated angle error. What's more,
acceleration/deceleration is inevitable in AUV operation.
And the usage of GNSS signal to correct the angles in
underwater is invalid for AHRS. Therefore, we need to
make reasonable use of low-cost sensors data to improve
navigation performance. Different from the traditional
angle correction, the proposed method aims to improve
the navigation performance by using data from low-cost
sensors directly, rather than only consider the
compensation of these lowcost sensors. As we mainly
focus on large-scale marine investigation and
detection, therefore, the sway of AUV in local area is
avoided as much as possible. Assuming that TCM/AHRS
is not affected by external environment
and the accuracy of them is high enough, the heading
angles of TCM/AHRS will be consistent with course
heading angles from GPS. In fact, the factor of external
interference and sensor errors are unavoidable.
So, only considering one factor, it is difficult to achieve
high-precision navigation. On the basis of these
problems, we adopt neural network to generate the full-noise model, which describe the relationship between the
sensors heading angles and course heading angles which
comes from GPS.


